FlashDiffusion: Fused Tiled Kernel Spectral Decomposition

Diffusion maps, and kernel methods more generally, provide an interpretable nonlinear spectral representation basis for geometric learning. In the geometric limit, small bandwidth, these matrices tend to be high rank and thus require materializing dense Gaussian kernels requires $O(N^2)$ memory. We introduce FlashDiffusion, a matrix-free method that evaluates dense Gaussian kernel blocks in fused GPU tiles and couples the eigensolver to an empirical $\beta$-flow that selects the finite-sample resolution scale. A continuation over sample size and bandwidth warm-starts increasingly expensive spectral solves from coarser resolutions.

==> figures/ramachandran.tex <==
% Ramachandran comparison figure.
% Expected in the same graphics search path as this fragment:
%   truth.png, m8.png, m256.png
%
% Preamble requirements:
%   \usepackage{pgfplots}
%   \usepgfplotslibrary{groupplots}
%   \pgfplotsset{compat=1.18}
%
% If this file and the PNGs live in a subdirectory (e.g. figures/), either add
%   \graphicspath{{figures/}}
% in the main document, or input the fragment with the import package.

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=3 by 1,
    horizontal sep=0.75cm,
    ylabels at=edge left,
    yticklabels at=edge left
  },
  scale only axis,
  width=0.255\textwidth,
  height=0.279\textwidth,
  xmin=-180,
  xmax=180,
  ymin=-180,
  ymax=180,
  xtick={-180,0,180},
  ytick={-180,0,180},
  xticklabels={$-180^{\circ}$,$0^{\circ}$,$180^{\circ}$},
  yticklabels={$-180^{\circ}$,$0^{\circ}$,$180^{\circ}$},
  xlabel={$\psi$},
  ylabel={$\phi$},
  axis on top,
  axis lines=box,
  tick align=outside,
  tick label style={font=\scriptsize},
  label style={font=\small},
  title style={font=\small},
  enlargelimits=false,
  clip=false
]

\nextgroupplot[title={(a) Reference}]
\addplot graphics[
  xmin=-180,xmax=180,
  ymin=-180,ymax=180
] {figures/truth.png};

\nextgroupplot[title={(b) 8 DMAP modes}]
\addplot graphics[
  xmin=-180,xmax=180,
  ymin=-180,ymax=180
] {figures/m8.png};

\nextgroupplot[title={(c) 256 DMAP modes}]
\addplot graphics[
  xmin=-180,xmax=180,
  ymin=-180,ymax=180
] {figures/m256.png};

\end{groupplot}
\end{tikzpicture}
\caption{Ramachandran distributions for alanine dipeptide. \textbf{(a)} Reference distribution, \textbf{(b)} reconstruction using 8 diffusion-map (DMAP) modes, and \textbf{(c)} reconstruction using 256 DMAP modes. The horizontal coordinate is the dihedral angle $\psi$ and the vertical coordinate is $\phi$; both span $[-180^{\circ},180^{\circ}]$, with $(\phi,\psi)=(0,0)$ at the center of each panel.}
\label{fig:alanine_anatomy}
\end{figure}

\input{figures/spectralres}

==> figures/spectralres.tex <==
% Spectral-resolution figure for alanine dipeptide.
% Expects AlanineDipeptide_traj.png in the same directory as this file
% (or on \graphicspath).
%
% Preamble requirements:
%   \usepackage{pgfplots}
%   \usepgfplotslibrary{groupplots}
%   \pgfplotsset{compat=1.18}

\begin{figure}[t]
\centering

% Matplotlib-like series colors used in the original plot.
\definecolor{spectralBlue}{RGB}{31,119,180}
\definecolor{spectralOrange}{RGB}{255,127,14}
\definecolor{spectralGreen}{RGB}{44,160,44}
\definecolor{spectralRed}{RGB}{214,39,40}

% All numerical data for panel (a), embedded so no external CSV is needed.
\pgfplotstableread[col sep=comma]{
m,phi_mae_traj,psi_mae_traj,joint_traj,phi_mae_rand,psi_mae_rand,joint_rand,cond_Gm
2,26.6896,15.5255,33.4886,27.0371,15.4093,33.6612,1.23099
4,12.0095,15.3419,21.4756,12.7291,15.2708,21.9019,1.27258
8,7.70748,14.9427,18.3073,7.92088,14.9675,18.443,3604.03
16,6.7314,9.64142,13.0685,6.93115,9.69588,13.2252,10380.6
32,5.93265,6.71444,9.98026,6.04413,6.65027,9.97478,18140.9
64,5.65941,5.13687,8.48853,5.75153,5.10989,8.5287,84775.1
128,5.26102,4.42413,7.60024,5.328,4.45284,7.67385,132625
256,4.85845,3.94828,6.91114,4.89654,3.95931,6.94705,185252
}\spectralResolutionData

\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=2 by 1,
    horizontal sep=1.25cm,
  },
  height=0.40\textwidth,
  tick label style={font=\scriptsize},
  label style={font=\small},
  title style={font=\small},
]

% ---------------------------------------------------------------------------
% (a) Spectral-resolution sweep
% ---------------------------------------------------------------------------
\nextgroupplot[
  width=0.47\textwidth,
  xmode=log,
  log basis x=2,
  xmin=1.7,
  xmax=300,
  ymin=3,
  ymax=28.5,
  xtick={2,4,8,16,32,64,128,256},
  xticklabels={$2^1$,$2^2$,$2^3$,$2^4$,$2^5$,$2^6$,$2^7$,$2^8$},
  xlabel={Number of diffusion modes $m$},
  ylabel={Held-out angular MAE (deg)},
  title={(a) Circular decoding at $\beta^\star=276.4$},
  legend style={
    at={(0.02,0.02)},
    anchor=south west,
    font=\scriptsize,
    draw=iclrTextColor!35,
    fill=iclrPageColor,
    fill opacity=0.90,
    text opacity=1,
    cells={anchor=west},
  },
]

\addplot+[
  spectralBlue,
  solid,
  mark=*,
  mark size=1.7pt,
  thick,
] table[x=m,y=phi_mae_traj]{\spectralResolutionData};
\addlegendentry{$\phi$ (held-out traj.)}

\addplot+[
  spectralOrange,
  solid,
  mark=*,
  mark size=1.7pt,
  thick,
] table[x=m,y=psi_mae_traj]{\spectralResolutionData};
\addlegendentry{$\psi$ (held-out traj.)}

\addplot+[
  spectralGreen,
  dashed,
  mark=square*,
  mark size=1.6pt,
  thick,
] table[x=m,y=phi_mae_rand]{\spectralResolutionData};
\addlegendentry{$\phi$ (random holdout)}

\addplot+[
  spectralRed,
  dashed,
  mark=square*,
  mark size=1.6pt,
  thick,
] table[x=m,y=psi_mae_rand]{\spectralResolutionData};
\addlegendentry{$\psi$ (random holdout)}

% Detected onset of the principal psi-resolution regime.
\draw[spectralOrange, densely dotted, thick]
  (axis cs:16,3) -- (axis cs:16,28.5)
  node[pos=0.96, anchor=east, rotate=90, font=\scriptsize]
  {$m_\psi=16$};

% Ambient E(3)-invariant feature dimension.
\draw[iclrTextColor!60, densely dotted, thick]
  (axis cs:80,3) -- (axis cs:80,28.5)
  node[pos=0.96, anchor=east, rotate=90, font=\scriptsize]
  {$D=80$};

% ---------------------------------------------------------------------------
% (b) Held-out Ramachandran surface and trajectory reconstruction
% ---------------------------------------------------------------------------
\nextgroupplot[
  width=0.40\textwidth,
  axis on top,
  xmin=-180,
  xmax=180,
  ymin=-180,
  ymax=180,
  xtick={-150,-100,-50,0,50,100,150},
  ytick={-150,-100,-50,0,50,100,150},
  xlabel={$\phi$ (deg)},
  ylabel={$\psi$ (deg)},
  title={(b) Held-out Ramachandran surface},
  enlargelimits=false,
]

\addplot graphics[
  xmin=-180,
  xmax=180,
  ymin=-180,
  ymax=180,
] {figures/AlanineDipeptide_traj.png};

\end{groupplot}

% ---------------------------------------------------------------------------
% Color bars for panel (b).
% The cropped raster contains both scalar fields, so these axes encode the
% scales used by the original plot without requiring the underlying point data.
% ---------------------------------------------------------------------------

% Random-holdout joint reconstruction error: 0--30 degrees.
\begin{axis}[
  hide axis,
  scale only axis,
  width=0pt,
  height=0pt,
  point meta min=0,
  point meta max=30,
  colormap={jointErrorMap}{
    rgb255(0cm)=(255,245,240);
    rgb255(1cm)=(252,174,145);
    rgb255(2cm)=(251,106,74);
    rgb255(3cm)=(203,24,29);
    rgb255(4cm)=(103,0,13)
  },
  colorbar,
  colorbar style={
    at={(group c2r1.east)},
    anchor=west,
    xshift=0.22cm,
    width=0.18cm,
    height=0.355\textwidth,
    ytick={0,5,10,15,20,25,30},
    ylabel={joint error (deg)},
    ylabel style={font=\scriptsize},
    tick label style={font=\scriptsize},
  },
]
\addplot[draw=none] coordinates {(0,0) (1,30)};
\end{axis}

% Ramachandran free energy: 0--8 k_B T.
\begin{axis}[
  hide axis,
  scale only axis,
  width=0pt,
  height=0pt,
  point meta min=0,
  point meta max=8,
  colormap/viridis,
  colorbar,
  colorbar style={
    at={(group c2r1.east)},
    anchor=west,
    xshift=1.00cm,
    width=0.18cm,
    height=0.355\textwidth,
    ytick={0,1,2,3,4,5,6,7,8},
    ylabel={$F/k_B T$},
    ylabel style={font=\scriptsize},
    tick label style={font=\scriptsize},
  },
]
\addplot[draw=none] coordinates {(0,0) (1,8)};
\end{axis}

\end{tikzpicture}

\caption{\textbf{Spectral resolution of alanine-dipeptide coordinates.}
\textbf{(a)} Mean absolute wrapped error for the backbone dihedrals $\phi$ and
$\psi$ as the number of retained diffusion modes $m$ increases. Solid curves
evaluate the completely held-out trajectory, while dashed curves evaluate
$5{,}000$ randomly held-out frames from the decoder-training trajectories. The
vertical markers indicate the ambient feature dimension $D=80$ and the detected
onset $m_\psi=16$ of the principal $\psi$-resolution regime.
\textbf{(b)} Held-out Ramachandran free-energy surface at
$\beta^\star=276.4$, with random-holdout frames colored by joint angular
reconstruction error and a strided segment of the decoded held-out trajectory
overlaid as a curve.}
\label{fig:alanine}
\end{figure}

